Why Watching Movie Tweets Won't Tell the Whole Story?

Data from Online Social Networks (OSNs) are providing analysts with an unprecedented access to public opinion on elections, news, movies etc. However, caution must be taken to determine whether and how much of the opinion extracted from OSN user data is indeed reflective of the opinion of the larger online population. In this work we study this issue in the context of movie reviews on Twitter and compare the opinion of Twitter users with that of the online population of IMDb and Rotten Tomatoes. We introduce new metrics to show that the Twitter users can be characteristically different from general users, both in their rating and their relative preference for Oscar-nominated and non-nominated movies. Additionally, we investigate whether such data can truly predict a movie's box-office success.

==> Conclusions.tex <==
\section{Conclusions}\label{concl}

This paper presents a study that compares data from Twitter to other online user population. We show that Twitter users are more positive in their reviews across most movies in comparison to other rating sites, like IMDb and Rotten Tomatoes. Moreover, compared to IMDb and Rotten Tomatoes users, the computed scores from Twitter users are slightly less positive for the Oscar-nominated best films but more positive for non-nominated films, which we quantify by introducing a few interesting information-theory inspired metrics  $\mathcal{P}$, $\mathcal{B}$, and $\mathcal{I}$, which together capture the ``bias" observed among Twitter users.  We also introduce a hype-approval metric $\mathcal{H}$, measured as a ratio of the total number of positive tweets the users make before and after watching a movie, and relate it with the ratings for the movie on IMDb or Rotten Tomatoes.  Finally, we show that scores computed from Twitter reviews and other online sites do not necessarily translate into predictable box-office. 
 
%The key conclusions from our study are:
%\begin{enumerate}
%\item Twitter users are more positive in their reviews across almost all movies, even in comparison to other online rating sites, like IMDb and Rotten Tomatoes.
%\item The scores from Twitter users are roughly the same as that of IMDb and Rotten Tomatoes for the Oscar-nominated best films, but Twitterers are especially likely to be much more positive about non-oscar nominated films when compared to the ratings from IMDb or Rotten Tomato users. We quantify this notion by defining a new metric that captures this ``bias" observed among Twitter users.
%\item We introduce a hype-satisfaction metric, measured as a ratio of the total number of positive tweets the users make before and after watching a movie, and correlate it with the ratings for the movie on IMDb or Rotten Tomato.
%\item Finally, we show that scores computed from Twitter reviews and other online sites do not necessarily translate into predictable box-office gains.
%\end{enumerate}

%Future work



==> Intro.tex <==
\section{Introduction}\label{Intro}

Online social networks (OSN) provide a rich repository of public opinion that are being used to analyze trends and predict outcomes. % of elections, movie box-office \cite{Diakopoulos,Asur}. 
%Today's online social networks (OSN) provide a rich repository of public opinion on various current events.  Not surprisingly, pollsters, analysts, and researchers alike have eagerly embraced the use of OSN data to analyze public sentiments, measure social influence, and even predict outcomes of elections and movie box-office \cite{Diakopoulos,Asur}. 
%While it is arguably true that passive monitoring of uninhibited exchanges among OSN users offers a valuable looking glass into the public psyche, 
But such practices have been criticized as it is unclear whether polling based on OSNs data can be extrapolated to the general population \cite{WSJ}. 
%because OSN users are not fully representative of the larger population \cite{WSJ}. 
Motivated by this need to evaluate the ``representativeness'' of OSN data, we report on a study of movie reviews in Twitter and compare them with other online rating sites (e.g., IMDb and Rotten Tomatoes) by introducing new metrics on inferrability ($\mathcal{I}$), positiveness ($\mathcal{P}$), bias ($\mathcal{B}$), and hype-approval ($\mathcal{H}$).

%The key contention is that the data from OSN users is not fully representative of the larger population, and hence should not be extrapolated to predict trends \cite{WSJ}.  In other words, are we currently \emph{reading too much into the OSN data?}.  
%Understanding this aspect is essential to both researchers, analysts, and marketing personnel as they need to be aware of the characteristic differences and bias that OSN users may exhibit when compared to the larger online user population.   
%Motivated by this need, we report on a study of Twitter user reviews of recent movies and compare them with other online rating websites, such as IMDb and Rotten Tomatoes.
%and to develop metrics that can quantify whether a data set is representative enough.   

Although the context of this work is movie reviews in Twitter, its scope extends to other product categories and social networks. Twitter is our choice for this study because marketers consider brand interaction and information dissemination as a major aspect of Twitter. %, perhaps much more so than other popular OSNs \cite{Baer}.
The focus on movies in this paper is also driven by two key factors: 

(a) \emph{Right in the Level of Interest:} Movies tend to generate a high interest among Twitter users as well as in other online user population (e.g., IMDb). 
%It has been studied that movies tend to generate a high interest among social network users (e.g., Twitterers) as well as the general online user population (e.g., IMDb).  This provides for a relatively direct comparison between the two user population for studying characteristic differences between these (partially overlapping) groups of netizens. 

(b) \emph{Right in Timing:} We collected Twitter data during Academy Award season (Oscars) to obtain a unique dataset to analyze characteristic differences between Twitter and IMDb or Rotten Tomatoes users in their reviews of Oscar-nominated versus non-nominated movies.  

%Motivate why we studied Twitter and focused on movies in particular.
%As a validation of this argument, critics have cited that as of May 2011, only 13\% of the adult online users are on 
%Therefore, a natural research question is whether we are \emph{reading too much into the OSN data?}.  
%In the context of movies, particularly around the time of the Oscars, we monitored several nominated and non-nominated movies (listed in Table \ref{movielist}) to seek answers the following questions:

We collected data from Twitter between February-March 2012 and manually labeled 10K tweets as training data for a set of classifiers based on SVM. We focus on the following questions to investigate whether Twitter data is sufficiently representative and indicative of future outcomes: 

$\bullet$ Are there more positive or negative reviews about movies on Twitter? 

$\bullet$ Do users tweet before or after watching a movie?

$\bullet$ How does the proportion of positive to negative reviews on Twitter compare to those from other movie rating sites (e.g., Rotten Tomatoes, IMDb)?

$\bullet$ Do the opinions of Twitter users about the Oscar-nominated and non-nominated movies differ quantitatively from these other rating sites?

$\bullet$ Does greater hype and positive reviews on Twitter directly translate to a higher rating for the movie in other rating sites?

$\bullet$ How well do reviews on Twitter and other online rating sites correspond to box-office gains or losses?
 
%Key highlights

The paper is organized as follows: Section \ref{rel-work} reviews related work. Section \ref{Method} discusses the data collection and classification techniques used. The results are reported in \ref{Results}, followed by conclusions in Section \ref{concl}. 



%List of contributions:
%
%1. Classifying tweets as after, Before, Current tweets  -why?
%
%2. Exploring whether Tweeters preference in movies is quantitatively different from general population. Important timing of Oscars. Taste difference between Oscar nominated and non-nominated movies in comparison to IMDB and RT users
%
%3. Do Tweeters tend to be more positive?  - Implications on marketing strategy
%
%4. Correlation between IMDB ratings and Hype sustenance on twitters to box office gains


%This work studies the issue in the context of movie reviews from Twitter and comparing these to outcomes on other sites  (e.g., Rotten Tomatoes, IMDB) that are accessed by a larger population of 
%\begin{itemize}
%\item Are there more positive or negative reviews about movies on Twitter?
%\item How does the proportion of positive to negative reviews on Twitter compare to those from other movie rating sites (e.g., Rotten Tomatoes, IMDB)?
%\item Do the opinions of Twitter users about the Oscar-nominated and non-nominated movies quantitatively differ from the general population ratings found in sites like Rotten Tomatoes and IMDB?
%\item Is there a correlation between a movie's hype sustainability on Twitter and its rating on other popular rating sites? 
%\end{itemize}






%Passively monitoring these uninhibited correspondence among friends and followers, and how information diffuses in the community  
 

%With the growth of e-commerce and OSNs, the impact of online positive and negative reviews have become an active area of research in both networking and management science communities. 
%Researchers have shown that ratings on sites like Amazon usually have a large number of very high and very low scores, which create \emph{U}-shaped histograms over the rating scale \cite{}. This observation was attributed to the ``brag-and-moan'' phenomenon among reviewers. But researchers have also suggested that due to risk-averseness among consumers, negative reviews tend to have a higher impact than positive reviews on purchase decisions \cite{}.  
%But the impact of such negative reviews will be greatly diminished if they are vastly outnumbered by positive reviews.  Hence it is natural to investigate whether positive reviews dominate in proportion to negative reviews on social networks like Twitter, where user comments diffuse freely and influence each other's decisions.  
% Arguably, understanding this aspect holds the key to developing successful marketing strategies and metrics for sellers and distributors in two significant ways: 
%
%(a) Instead of focusing on reducing the negative ratings from dissatisfied customers, should the marketing be more geared towards enhancing their already high proportion of positive reviews on social networks?   
%
%(b) Conversely, how should the count of the proportion of positive reviews on social networks be scaled down to forecast the actual ratings for the general population? 
%
%[[Add Paragraphs]]

%Introduce metric of ratio of TwitterP/N to IMDB rating.

%Let's plot before negative (handmarked in those 10K labels) and then with m/c learning.

%In the context of movies, particularly around the time of the Oscars, we monitored several nominated and non-nominated movies (listed in Table \ref{movielist}) to seek answers the following questions:
%\begin{itemize}
%\item Are there more positive or negative reviews about movies on Twitter?
%%\item Do Twitter users tend to be more positively or negatively biased in their movie reviews in comparison to other movie rating sites (e.g., Rotten Tomatoes, IMDB)?
%\item How does the proportion of positive versus negative reviews on Twitter compare to those from other movie rating sites (e.g., Rotten Tomatoes, IMDB)?
%\item Do the opinions of Twitter users about the Oscar-nominated and non-nominated movies quantitatively differ from the general population ratings found in sites like Rotten Tomatoes and IMDB?
%\item Are the movies that receive more positive reviews on Twitter during the Oscar season also tend to do well in the Oscar night?
%\item Is there a correlation between the hype that a movie generates on Twitter and its rating on other popular rating sites? 
%\end{itemize}
% xs


==> Related-work.tex <==
\section{Related Work}\label{rel-work}

%Over the last few years, several researchers have focused on various aspects of OSN data and their applied them in deriving interesting insights. 
This work complements earlier works in three related topics: (a) OSNs as a medium of information dissemination, (b) sentiments analysis, and (c) Twitter's role in predicting movies box-office.

\indent{\bf Network Influence.}
Several works have reported on how OSN users promote viral information dissemination \cite{Leskovec} and create powerful electronic ``word-of-mouth" (WoM) effects \cite{Jansen} through tweets. 
\cite{Krish,Mislove} study these tweets to identify social interaction patterns, user behavior, and network growth. Instead, we focus on the sentiment expressed in these tweets on popular new movies and their ratings.

%User tweets from Twitter have been used to identify social interaction patterns, user behaviors, geographic growth patterns, and the size of the network \cite{Krish}. 
%\cite{Jansen} reported on the power of tweets in becoming a electronic ``word-of-mouth", while \cite{Hansen,Leskovec} studied the influence of network users in promoting virality in OSNs. 
%The role of Twitter as a social media for fast disseminating of information was analyzed in the aftermath of earthquakes was considered in \cite{Sakaki}.

\indent{\bf Sentiment Analysis \& Box-office Forecasting.}
Researchers have mined Twitter dataset to analyze public reaction to various events, from election debate performance \cite{Diakopoulos} to movie box-office predictions on the release day \cite{Asur}. In contrast, we improve on the training and classification techniques, and specifically focus on developing new metrics to ascertain whether opinions of Twitter users are sufficiently representative of the general online population of sites like IMDb and Rotten Tomatoes. Additionally, we also revisit the issue of how well factors like hype and satisfaction reported in the user tweets can be translated to online ratings and eventual box-office sales.



%However, these work does not focus on studying whether the Twitter users are sufficiently representative of the general online population on other sites, or how the hype and audience satisfaction reported in tweets translate in to movie ratings or eventual box-office sales.  

%Researchers have also mined Twitter dataset for identifying user sentiments and popular trends. For example, \cite{Diakopoulos} reported on using tweets to analyze reactions to election debate performance, \cite{Connor} linked text sentiments to create time series on public opinion. Others have focused on improving the performance of sentiment analysis techniques \cite{Barbosa,Pak}. 
%An overview of various works on topic tracking and sentiment analysis in Twitter is presented in [Mejova].

%\indent{\bf Box-office Forecasting.}
%An early work on forecasting opening box-office sales to pre-release hype on Twitter was undertaken by \cite{Asur}.  Extracting text and metadata from tweets to forecast box-office sales using regression has also been explored by \cite{Joshi}.  However, these work does not focus on studying whether the Twitter users are sufficiently representative of the general online population on other sites, or how the hype and audience satisfaction reported in tweets translate in to movie ratings or eventual box-office sales.

%Several works have reported on how OSN users promote viral information dissemination \cite{Leskovec} and create powerful electronic ``word-of-mouth" (WoM) effects \cite{Jansen} through tweets.  The user sentiment expressed in these tweets have been used to identify public reactions to election debates \cite{Diakopoulos}, movie box-office \cite{Asur} etc. 

